Object-Aware Query Perturbation for Cross-Modal Image-Text Retrieval

The pre-trained vision and language (V\&L) models have substantially improved the performance of cross-modal image-text retrieval. In general, however, V\&L models have limited retrieval performance for small objects because of the rough alignment between words and the small objects in the image. In contrast, it is known that human cognition is object-centric, and we pay more attention to important objects, even if they are small. To bridge this gap between the human cognition and the V\&L model's capability, we propose a cross-modal image-text retrieval framework based on ``object-aware query perturbation.'' The proposed method generates a key feature subspace of the detected objects and perturbs the corresponding queries using this subspace to improve the object awareness in the image. In our proposed method, object-aware cross-modal image-text retrieval is possible while keeping the rich expressive power and retrieval performance of existing V\&L models without additional fine-tuning. Comprehensive experiments on four public datasets show that our method outperforms conventional algorithms. Our code is publicly available at \url{https://github.com/NEC-N-SOGI/query-perturbation}.

==> supp_tab/eccv_supp_tab1.tex <==

\begin{table}
    \centering
\caption{Caption}
\label{tab:my_label}
    \begin{tabular}{lrrrrrrrrrrr}
    \toprule
         &  \textasciitilde 10\%&  \textasciitilde 20\%&  \textasciitilde 30\%&  \textasciitilde 40\%&  \textasciitilde 50\%&  \textasciitilde 60\%&  \textasciitilde 70\%&  \textasciitilde 80\%& \textasciitilde 90\% &\textasciitilde 100\% &mR@1\\
    \midrule
         &  \multicolumn{11}{c}{Flickr-30K T2I}\\
    \midrule
         BLIP2&  81.33 &  85.00 &  90.11 &  87.59 &  88.92 &  91.29 &  90.89 &  90.67 &  92.56 & 90.38 
&88.75 
\\
         ~~w/Q-Pert.(E)&  84.00 &  85.00 &  90.97 &  87.41 &  89.19 &  91.00 &  90.89 &  90.67 &  92.56 & 90.13 
&89.10 
\\
         ~~w/Q-Pert.(D)&  84.00 &  85.67 &  90.11 &  87.59 &  89.32 &  91.29 &  90.36 &  90.44 &  92.31 & 90.77 
&89.11 
\\
    \midrule
         &  \multicolumn{11}{c}{Flickr-30K I2T}\\
    \midrule
         BLIP2
&  93.33 &  98.33 &  97.85 &  96.30 &  99.32 &  96.43 &  96.43 &  97.78 &  98.72 & 98.08 
&97.23 
\\
 ~~w/Q-Pert.(E)
& 93.33 & 98.33 & 97.85 & 98.15 & 99.32 & 97.14 & 96.43 & 97.78 & 98.72 & 98.72 
&97.55 
\\
 ~~w/Q-Pert.(D)& 93.33 & 98.33 & 96.77 & 97.22 & 99.32 & 97.14 & 96.43 & 97.78 & 98.72 & 98.08 
&97.29 

\\
    \midrule
        & \multicolumn{11}{c}{COCO-5K T2I}\\
    \midrule
 BLIP2
& 59.87 & 64.37 & 66.66 & 72.11 & 75.01 & 72.16 & 75.93 & 75.45 & 76.26 & 77.94 
&71.09 
\\
 ~~w/Q-Pert.(E)
& 60.17 & 64.39 & 66.66 & 72.11 & 75.20 & 72.16 & 75.84 & 75.35 & 76.26 & 78.00 
&71.14 
\\
 ~~w/Q-Pert.(D)& 60.09 & 64.39 & 67.03 & 71.96 & 75.48 & 71.98 & 75.93 & 75.25 & 76.40 & 77.73 
&71.15 
\\
    \midrule
        & \multicolumn{11}{c}{COCO-5K I2T}\\
    \midrule
 BLIP2
& 80.18 & 82.50 & 81.61 & 88.24 & 90.70 & 87.65 & 91.59 & 92.57 & 89.93 & 91.51 
&87.43 
\\
~~w/Q-Pert.(E)
& 80.93 & 82.39 & 82.23 & 88.05 & 90.70 & 87.35 & 92.04 & 92.08 & 89.93 & 91.51 
&87.52 
\\
 ~~w/Q-Pert.(D)& 79.85 & 82.73 & 82.38 & 88.24 & 90.70 & 87.35 & 92.48 & 92.57 & 91.37 & 91.51 
&87.69 
\\
    \midrule
        & \multicolumn{11}{c}{Flickr-FG T2I}\\
    \midrule
BLIP2&  85.33 &  90.00 &  92.69 &  90.93 &  92.16 &  93.43 &  93.04 &  93.11 &  95.64 & 92.31 
&91.79 
\\
         ~~w/Q-Pert.(E)&  86.67 &  90.67 &  92.90 &  91.11 &  92.57 &  93.00 &  92.86 &  92.44 &  95.38 & 92.69 
&91.98 
\\
         ~~w/Q-Pert.(D)&  86.67 &  90.67 &  92.47 &  91.30 &  92.30 &  93.43 &  92.86 &  93.11 &  95.38 & 92.95 
&92.06 
\\
    \midrule
         &  \multicolumn{11}{c}{Flickr-FG I2T}\\
    \midrule
         BLIP2
&  100.00 &  100.00 &  98.92 &  99.07 &  99.32 &  97.86 &  98.21 &  96.67 &  100.00 & 97.44 
&98.50 
\\
 ~~w/Q-Pert.(E)
& 100.00 & 100.00 & 98.92 & 98.15 & 99.32 & 97.86 & 98.21 & 98.89 & 100.00 & 97.44 
&98.60 
\\
 ~~w/Q-Pert.(D)& 100.00 & 100.00 & 98.92 & 99.07 & 99.32 & 97.86 & 98.21 & 97.78 & 100.00 & 97.44 
&98.60 
\\
    \midrule
        & \multicolumn{11}{c}{COCO-FG T2I}\\
    \midrule
 BLIP2
& 63.93 & 68.25 & 71.65 & 77.43 & 79.12 & 77.96 & 81.33 & 79.80 & 81.58 & 80.85 
&75.71 
\\
 ~~w/Q-Pert.(E)
& 64.00 & 68.39 & 71.59 & 77.46 & 79.35 & 77.96 & 81.06 & 80.30 & 81.58 & 80.80 
&75.77 
\\
 ~~w/Q-Pert.(D)& 64.06 & 68.41 & 71.65 & 77.46 & 79.21 & 78.02 & 81.24 & 80.30 & 81.29 & 80.95 
&75.78 
\\
    \midrule
        & \multicolumn{11}{c}{COCO-FG I2T}\\
    \midrule
 BLIP2
& 81.18 & 84.94 & 85.94 & 90.07 & 92.79 & 92.90 & 92.04 & 94.06 & 92.09 & 94.43 
&89.83 
\\
~~w/Q-Pert.(E)
& 81.93 & 85.17 & 85.94 & 90.26 & 92.79 & 93.21 & 91.59 & 93.56 & 92.81 & 94.43 
&89.98 
\\
 ~~w/Q-Pert.(D)& 81.27 & 84.70 & 86.24 & 90.26 & 93.95 & 92.28 & 92.04 & 93.56 & 92.09 & 94.43 
&89.87 
\\
\bottomrule
    \end{tabular}
    
    
\end{table}

==> supp_tab/eccv_supp_tab2.tex <==

\begin{table}
\caption{Hoge}
    \begin{minipage}[c]{.5\hsize}
        \centering
        
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{scale}\\
        \midrule
            &&  2 &  4&  6&  8& 10\\
        \midrule
            &$\bar{S}$ &  81.33&  82.67&  81.33&  80& 81.33
\\
            &1-$\bar{S}$ &  82.67&  82.67&  80&  81.33& 84
\\
            &$\bar{S}$-0.5 &  81.33&  81.33&  81.33&  82.67& 82.67
\\
            &0.5-$\bar{S}$&  81.33&  82.67&  81.33&  81.33& 81.33
\\
            &constant&  82.67&  81.33&  81.33&  81.33& 84
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1 small(10\%)}
    \end{minipage}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{scale}\\
        \midrule
            &&  2 &  4&  6&  8& 10\\
        \midrule
            &$\bar{S}$ &  88.73&  88.65&  88.67&  88.67& 88.77
\\
            &1-$\bar{S}$ &  88.85&  88.63&  88.63&  88.93& 88.62
\\
            &$\bar{S}$-0.5 &  88.69&  88.41&  88.75&  88.46& 88.52
\\
            &0.5-$\bar{S}$&  88.53&  88.8&  88.81&  88.72& 88.63
\\
            &constant&  88.63&  88.95&  88.93&  88.67& 88.76
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1}
    \end{minipage}
    \label{tab:scale_sensitivity}
\end{table}


\begin{table}
    \caption{Hoge}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{Contribution ratio
}\\
        \midrule
            &&  0.80&  0.85&  0.90&  0.95& 0.99
\\
        \midrule
            &$\bar{S}$ &  81.33&  81.33&  81.33&  81.33& 
82.67
\\
            &1-$\bar{S}$ &  81.33&  84&  84&  82.67& 
81.33
\\
            &$\bar{S}$-0.5 &  81.33&  80&  80&  80& 
81.33
\\
            &0.5-$\bar{S}$&  81.33&  81.33&  80&  81.33& 
81.33
\\
            &constant&  81.33&  81.33&  85.33&  82.67& 84
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1 small(10\%)}
    \end{minipage}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{Contribution ratio
}\\
        \midrule
            &&  0.80&  0.85&  0.90&  0.95& 0.99
\\
        \midrule
            &$\bar{S}$ &  88.6&  88.6&  88.75&  88.59& 
88.77
\\
            &1-$\bar{S}$ &  88.84&  89.16&  88.84&  88.81& 
88.62
\\
            &$\bar{S}$-0.5 &  88.83&  88.46&  88.43&  88.49& 
88.52
\\
            &0.5-$\bar{S}$&  88.78&  88.75&  88.51&  88.67& 
88.63
\\
            &constant&  88.57&  88.67&  89.14&  88.7& 88.76
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1}
    \end{minipage}    
    \label{tab:scale_sensitivity}
\end{table}

==> supp_tab/eccv_supp_tab3.tex <==

\begin{table}
    \centering
\caption{Bold: the best result in each column. Underscore: the best result in each row}
\label{tab:my_label}
    \begin{tabular}{llrrrrrrrcc}
\toprule
 & & Steep& & & & & & Smooth& &\\
          &var&  1 &  6&  12&  24&  48&  96&  192&  & \\
\midrule
 & \multicolumn{8}{c}{Flickr}& &\\
\bottomrule
 org Q-Pert.& & \multicolumn{7}{c}{89.54}& &\\
\hdashline
          &Former&  89.70 &  \second{89.80}&  \first{89.78}&  \first{89.64}&  89.54 &  89.58 &  89.54 
&  & \\
          R@1&Middle&  89.74 &  \first{\second{89.82}}&  89.74 &  89.44 &  89.56 &  89.52 &  89.54 
&  & \\
          &Latter&  \first{\second{89.78}}&  89.66 &  89.64 &  89.42 &  \first{89.74}&  \first{89.60}&  \first{89.60}&  & \\
\bottomrule
 org Q-Pert.& & \multicolumn{7}{c}{88.54}& &\\
\hdashline
          &Former
&  88.70 &  \second{88.96}&  88.80 &  \first{88.80}&  88.70 &  \first{88.64}&  88.52 
&  & \\
          mR@1&Middle
&  \first{88.90}&  \first{\second{88.99}}&  \first{88.97}&  88.45 &  88.60 &  88.50 &  88.50 
&  & \\
          &Latter&  \second{88.73}&  88.59 &  88.44 &  88.22 &  \first{\second{88.73}}&  88.60 &  \first{88.59}&  & \\
\midrule
 & \multicolumn{8}{c}{Flickr-FG}& &\\
\midrule
 org Q-Pert.& & \multicolumn{7}{c}{92.16}& &\\
\hdashline
 & Former
& \first{92.60}& 92.44& \first{92.56}& 92.44& 92.52& \first{\second{92.68}}& \first{92.60}& &\\
 & Middle
& 92.48& \first{92.58}& 92.48& \first{\second{92.72}}& \first{92.68}& 92.48& 92.46
& &\\
 & Latter& 92.42& 92.4& 92.46& 92.54& 92.54& \second{92.66}& 92.52
& &\\
\midrule
 org Q-Pert.& & \multicolumn{7}{c}{91.74}& &\\
\hdashline
 & Former
& \first{92.03}& 91.76& \first{91.81}& 91.72& 91.95& \first{\second{92.10}}& \first{92.03}& &\\
 & 
Middle
& 91.74& \first{91.86}& 91.75& \first{\second{92.14}}& \first{92.10}& 91.93& 91.77
& &\\
 & Latter& 91.73& 91.62& 91.71& 91.80& 91.78& \second{91.93}& 91.84
& &\\
\bottomrule
    \end{tabular}
    
    
\end{table}

==> tables/all_ablations.tex <==

\begin{table}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{scale}\\
        \midrule
            &&  2 &  4&  6&  8& 10\\
        \midrule
            &$\bar{S}$ &  81.33&  82.67&  81.33&  80& 81.33
\\
            &1-$\bar{S}$ &  82.67&  82.67&  80&  81.33& 84
\\
            &$\bar{S}$-0.5 &  81.33&  81.33&  81.33&  82.67& 82.67
\\
            &0.5-$\bar{S}$&  81.33&  82.67&  81.33&  81.33& 81.33
\\
            &constant&  82.67&  81.33&  81.33&  81.33& 84
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1 small(10\%)}
    \end{minipage}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{scale}\\
        \midrule
            &&  2 &  4&  6&  8& 10\\
        \midrule
            &$\bar{S}$ &  88.73&  88.65&  88.67&  88.67& 88.77
\\
            &1-$\bar{S}$ &  88.85&  88.63&  88.63&  88.93& 88.62
\\
            &$\bar{S}$-0.5 &  88.69&  88.41&  88.75&  88.46& 88.52
\\
            &0.5-$\bar{S}$&  88.53&  88.8&  88.81&  88.72& 88.63
\\
            &constant&  88.63&  88.95&  88.93&  88.67& 88.76
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1}
    \end{minipage}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{scale}\\
        \midrule
            &&  2 &  4&  6&  8& 10\\
        \midrule
            &$\bar{S}$ &  89.76&  89.56&  89.68&  89.72& 89.66
\\
            &1-$\bar{S}$ &  89.74&  89.52&  89.68&  89.78& 89.68
\\
            &$\bar{S}$-0.5 &  89.72&  89.56&  89.76&  89.5& 89.52
\\
            &0.5-$\bar{S}$&  89.72&  89.84&  89.66&  89.72& 89.7
\\
            &constant&  89.66&  89.74&  89.82&  89.72& 89.44
\\
        \bottomrule
        \end{tabular}
        \subcaption{mean R@1}
    \end{minipage}
    \caption{Hoge}
    \label{tab:scale_sensitivity}
\end{table}


\begin{table}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{Contribution ratio
}\\
        \midrule
            &&  0.80&  0.85&  0.90&  0.95& 0.99
\\
        \midrule
            &$\bar{S}$ &  81.33&  81.33&  81.33&  81.33& 
82.67
\\
            &1-$\bar{S}$ &  81.33&  84&  84&  82.67& 
81.33
\\
            &$\bar{S}$-0.5 &  81.33&  80&  80&  80& 
81.33
\\
            &0.5-$\bar{S}$&  81.33&  81.33&  80&  81.33& 
81.33
\\
            &constant&  81.33&  81.33&  85.33&  82.67& 84
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1 small(10\%)}
    \end{minipage}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{Contribution ratio
}\\
        \midrule
            &&  0.80&  0.85&  0.90&  0.95& 0.99
\\
        \midrule
            &$\bar{S}$ &  88.6&  88.6&  88.75&  88.59& 
88.77
\\
            &1-$\bar{S}$ &  88.84&  89.16&  88.84&  88.81& 
88.62
\\
            &$\bar{S}$-0.5 &  88.83&  88.46&  88.43&  88.49& 
88.52
\\
            &0.5-$\bar{S}$&  88.78&  88.75&  88.51&  88.67& 
88.63
\\
            &constant&  88.57&  88.67&  89.14&  88.7& 88.76
\\
        \bottomrule
        \end{tabular}
        \subcaption{R@1}
    \end{minipage}
    \begin{minipage}[c]{.5\hsize}
        \centering
        \begin{tabular}{llrrrrr}
        \toprule
            && \multicolumn{5}{c}{Contribution ratio}\\
        \midrule
            &&  0.80&  0.85&  0.90&  0.95& 0.99\\
        \midrule
            &$\bar{S}$ &  89.64&  89.68&  89.76&  89.62& 89.66
\\
            &1-$\bar{S}$ &  89.94&  90&  89.62&  89.82& 89.68
\\
            &$\bar{S}$-0.5 &  89.84&  89.58&  89.54&  89.68& 89.52
\\
            &0.5-$\bar{S}$&  89.8&  89.86&  89.74&  89.74& 89.7
\\
            &constant&  89.56&  89.68&  89.82&  89.64& 89.44
\\
        \bottomrule
        \end{tabular}
        \subcaption{mean R@1}
    \end{minipage}
    \caption{Hoge}
    \label{tab:scale_sensitivity}
\end{table}
